Visual Based Navigation of Mobile Robots

We have developed an algorithm to generate a complete map of the traversable region for a personal assistant robot using monocular vision only. Using multiple taken by a simple webcam, obstacle detection and avoidance algorithms have been developed. Simple Linear Iterative Clustering (SLIC) has been used for segmentation to reduce the memory and computation cost. A simple mapping technique using inverse perspective mapping and occupancy grids, which is robust, and supports very fast updates has been used to create the map for indoor navigation.

==> Past.tex <==
\chapter{Previous Work}
\begin{itemize}
    \item Developing the algorithms to be used
    \item Simple Linear Iterative Clustering (SLIC) of images
    \item Histogram Sampling
    \item Accessing individual superpixel
    \item Safe zone histogram sampling
\end{itemize}
